An Improved Parameterized Algorithm for Treewidth

We give an algorithm that takes as input an $n$-vertex graph $G$ and an integer $k$, runs in time $2^{O(k^2)} n^{O(1)}$, and outputs a tree decomposition of $G$ of width at most $k$, if such a decomposition exists. This resolves the long-standing open problem of whether there is a $2^{o(k^3)} n^{O(1)}$ time algorithm for treewidth. In particular, our algorithm is the first improvement on the dependency on $k$ in algorithms for treewidth since the $2^{O(k^3)} n^{O(1)}$ time algorithm given by Bodlaender and Kloks [ICALP 1991] and Lagergren and Arnborg [ICALP 1991]. We also give an algorithm that given an $n$-vertex graph $G$, an integer $k$, and a rational $\varepsilon \in (0,1)$, in time $k^{O(k/\varepsilon)} n^{O(1)}$ either outputs a tree decomposition of $G$ of width at most $(1+\varepsilon)k$ or determines that the treewidth of $G$ is larger than $k$. Prior to our work, no approximation algorithms for treewidth with approximation ratio less than $2$, other than the exact algorithms, were known. Both of our algorithms work in polynomial space.

==> Preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}
\pdfoutput=1

\usepackage{microtype}
\usepackage{mdframed}
\usepackage{csquotes}
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}
\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{graphicx,tikz-cd}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage[disable]{todonotes}
%%%%%
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{makecell}
\usepackage{thmtools, thm-restate}
\usepackage{thm-autoref}
 \usepackage{mathdots}
%\usepackage{wrapfig}
\usepackage{multirow}
%\usetikzlibrary{cd}
\usepackage{chngcntr}
\usepackage{apptools}
\AtAppendix{\counterwithin{lemma}{section}}




\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}[lemma]{Claim}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{observation}[lemma]{Observation}
\newtheorem{proposition}[lemma]{Proposition}
%\newtheorem{corollary}[lemma]{Corollary}
%\newtheorem{redrule}[lemma]{Reduction Rule}
%\newtheorem{remark}[lemma]{Remark}
%\newtheorem{reduction}[lemma]{Reduction Rule}
%\newtheorem{conjecture}[lemma]{Conjecture}


\date{}

\newcommand{\defparsproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameters:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}


\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hypertexnames = false,
                 hyperfigures
                 ]{hyperref}
\usepackage[nameinlink]{cleveref}
\crefname{observation}{Observation}{Observations}
\crefname{claim}{Claim}{Claims}
%\crefname{redrule}{Reduction Rule}{Reduction Rules}

\newcommand{\floor}[1]{\lfloor {#1} \rfloor}
\newcommand{\Floor}[1]{\left\lfloor {#1} \right\rfloor}
\newcommand{\ceil}[1]{\lceil {#1}\rceil}
\newcommand{\Ceil}[1]{\left\lceil {#1}\right\rceil}
\newcommand{\eps}{\varepsilon}
\newcommand{\OO}{\mathcal{O}}

\newcommand{\torso}{\texttt{torso}}
\newcommand{\flow}{\texttt{flow}}
\newcommand{\bag}{\texttt{bag}}
\newcommand{\cmp}{\texttt{cmp}}
\newcommand{\desc}{\texttt{desc}}
\newcommand{\ps}{\mathcal{P}}
\newcommand{\fw}{\lambda}
\newcommand{\mcliq}{\otimes}
\newcommand{\ins}{\mathcal{I}}
\newcommand{\reach}{R}
\newcommand{\reachn}{R^N}
\newcommand{\allw}{\hat{W}}
\newcommand{\rescliqs}{\triangleleft}
\newcommand{\mergcliqs}{\times}
\newcommand{\addv}{+}
\newcommand{\vertsz}{\texttt{gs}}
\newcommand{\fld}{\phi}
\newcommand{\ow}{\overline{W}}
\newcommand{\flp}{\texttt{flp}}
\newcommand{\og}{G_O}
\newcommand{\ogw}{W_O}

\newcommand{\pstw}{\textsc{Partitioned Subset Treewidth}\xspace}
\newcommand{\stw}{\textsc{Subset Treewidth}\xspace}

\newcommand{\no}{\textsf{NO}\xspace}
\newcommand{\invalid}{\textsf{INVALID}\xspace}

\newcommand{\ql}{\delta}
\newcommand{\potl}{\phi}
\newcommand{\pots}{\mu}
\newcommand{\tcbasea}{16}
\newcommand{\kb}{64}

\newcommand{\cq}{\texttt{cq}}

\newcommand{\ctc}{\texttt{ctc}}
\newcommand{\tc}{\texttt{tc}}
